DynamicVAE: Decoupling Reconstruction Error and Disentangled Representation Learning

This paper challenges the common assumption that the weight $\beta$, in $\beta$-VAE, should be larger than $1$ in order to effectively disentangle latent factors. We demonstrate that $\beta$-VAE, with $\beta < 1$, can not only attain good disentanglement but also significantly improve reconstruction accuracy via dynamic control. The paper removes the inherent trade-off between reconstruction accuracy and disentanglement for $\beta$-VAE. Existing methods, such as $\beta$-VAE and FactorVAE, assign a large weight to the KL-divergence term in the objective function, leading to high reconstruction errors for the sake of better disentanglement. To mitigate this problem, a ControlVAE has recently been developed that dynamically tunes the KL-divergence weight in an attempt to control the trade-off to more a favorable point. However, ControlVAE fails to eliminate the conflict between the need for a large $\beta$ (for disentanglement) and the need for a small $\beta$. Instead, we propose DynamicVAE that maintains a different $\beta$ at different stages of training, thereby decoupling disentanglement and reconstruction accuracy. In order to evolve the weight, $\beta$, along a trajectory that enables such decoupling, DynamicVAE leverages a modified incremental PI (proportional-integral) controller, and employs a moving average as well as a hybrid annealing method to evolve the value of KL-divergence smoothly in a tightly controlled fashion. We theoretically prove the stability of the proposed approach. Evaluation results on three benchmark datasets demonstrate that DynamicVAE significantly improves the reconstruction accuracy while achieving disentanglement comparable to the best of existing methods. The results verify that our method can separate disentangled representation learning and reconstruction, removing the inherent tension between the two.

==> impact.tex <==
\section*{Broader Impact}
The proposed ControlVAE is able to precisely control the value of KL-divergence, which can be widely used in various applications, such as text generation and disentangled representation learning. The proposed approach has a great impact on both industry and academia. Due to the its good performance on text generation, our model has be applied and deployed a famous Chinese E-commerce platform (anonymous due to double blind) to generates diverse and personalized item descriptions to different customers when shopping online. In addition, researchers from some famous companies and institutions, such as Sony, IBM research, University of Arkansas and Instadeep, are very interested in our method and contacted us to request the source code.

As with most generative modeling, ControlVAE is likely to be used to generate fake reviews on E-commerce platforms, such as Yelp and Amazon. Despite of that, our method with dynamic learning provides a new way to generate diverse text and learn disentangled factors for future research.
